Simple Stochastic and Online Gradient Descent Algorithms for Pairwise Learning

Pairwise learning refers to learning tasks where the loss function depends on a pair of instances. It instantiates many important machine learning tasks such as bipartite ranking and metric learning. A popular approach to handle streaming data in pairwise learning is an online gradient descent (OGD) algorithm, where one needs to pair the current instance with a buffering set of previous instances with a sufficiently large size and therefore suffers from a scalability issue. In this paper, we propose simple stochastic and online gradient descent methods for pairwise learning. A notable difference from the existing studies is that we only pair the current instance with the previous one in building a gradient direction, which is efficient in both the storage and computational complexity. We develop novel stability results, optimization, and generalization error bounds for both convex and nonconvex as well as both smooth and nonsmooth problems. We introduce novel techniques to decouple the dependency of models and the previous instance in both the optimization and generalization analysis. Our study resolves an open question on developing meaningful generalization bounds for OGD using a buffering set with a very small fixed size. We also extend our algorithms and stability analysis to develop differentially private SGD algorithms for pairwise learning which significantly improves the existing results.

==> miscellaneous.tex <==
\section{A Pair at a Time}

\begin{algorithm}[ht!]
\caption{Differentially Private Stochastic Gradient Descent for Pairwise Learning\label{alg:dp-sgd-4}}
\begin{algorithmic}[1]
\STATE {\bf Inputs:} Dataset $S = \{\zbf_i: i=1,\ldots, n\}$, loss function $\ell$ with Lipschitz constant $L$, learning rates $\{\eta_t\}_{t=1}^T$, %the convex set $\Omega \subseteq \mathcal{B}(0,R)$, 
privacy parameter $\epsilon$, $\delta$ and constant $\beta$.
\STATE \textbf{Set:} $\wbf_1=\mathbf{0}$ 
\STATE Compute $\sigma^2 = \frac{56L^2T}{\beta n^2\epsilon}\Big(\frac{\log(1/\delta)}{(1-\beta)\epsilon} + 1\Big)$
\FOR{$t=1,\ldots,T-1$}
\STATE Select $(i_{t},j_{t})$ from the uniform distribution over the set $\{(i,j):i,j\in [n], i \neq j\}$ 
\STATE Sample noise $\ubf_t \sim \ncal(0, \sigma^2 \mathbf{I})$
\STATE $\wbf_{t+1} = \proj_\wcal\big(\wbf_t - \eta_t (\nabla \ell(\wbf_t; \zbf_{i_{t}}, \zbf_{j_t}) + \ubf_t)\big)$
\ENDFOR
\STATE {\bf Outputs:} $\wbf_T$ 
\end{algorithmic}
\end{algorithm}


\begin{theorem}
Suppose the loss function $\ell$ is $L$-Lipschitz, then Algorithm~\ref{alg:dp-sgd-4} satisfies $(\epsilon, \delta)$-DP when $\ubf_t \sim \ncal(0, \sigma^2 \mathbf{I})$, if there exists $\beta \in(0,1)$ such that $\sigma^2 \ge 2.68 L^2$ 	and $\lambda-1\le \frac{\sigma^2}{6L^2} \log(\frac{n}{2\lambda  (1+\sigma^2/4L^2 )})$ with $\lambda=\frac{\log(1/\delta)}{(1-\beta)\epsilon}+1$.
\end{theorem}

\begin{proof}
Let $\mathcal{A}_t=\mathcal{M}_t+\ubf_t$ with $\mathcal{M}_t=\nabla \ell(\wbf_t; \zbf_{i_{t}}, \zbf_{j_t}) $. Since $\ell$ is $L$-Lipschitz, then for any $\wbf_t\in \mathbb{R}$ and any $(\zbf_{i_{t}}, \zbf_{j_t})$ and $(\zbf_{i_{t}}', \zbf_{j_t}')$, there holds
$$\|\nabla \ell(\wbf_t; \zbf_{i_{t}}, \zbf_{j_t}) -\nabla \ell(\wbf_t; \zbf_{i_{t}}', \zbf_{j_t}') \|_2\le 2L.$$
Therefore, the $\ell_2$-sensitivity of $\mathcal{A}_t$ is $2L$ for any $t=1,\ldots, T-1$. Let 
$$\sigma^2=\frac{56L^2 T}{\beta n^2 \epsilon}\big( \frac{\log(1/\delta)}{(1-\beta)\epsilon} + 1\big), $$
then Lemma 2 in \citet{liang2020exploring} with subsampling rate $p=\frac{2}{n}$ implies $\mathcal{A}_t$ satisfies $\big(\lambda, \frac{\lambda \beta \epsilon}{T( \frac{\log(1/\delta)}{(1-\beta)\epsilon} +1)}\big)$-RDP, if 
\begin{equation}\label{eq:rdp-condition-1}
	\sigma^2\ge 2.68 L^2
\end{equation}
and 
\begin{equation}\label{eq:rdp-condition-2}
	\lambda-1\le \frac{\sigma^2}{6L^2}\log\Big(\frac{n}{2\lambda(1+\sigma^2/4L^2)}\Big). 
\end{equation}
Now, let $\lambda=\frac{\log(1/\delta)}{(1-\beta)\epsilon}+1$, then we have $\mathcal{A}_t$ satisfies $\big( \frac{\log(1/\delta)}{(1-\beta)\epsilon}+1, \frac{\beta \epsilon}{T} \big)$-RDP. The post processing property of RDP implies that $\wbf_{t+1}$ also satisfies $\big( \frac{\log(1/\delta)}{(1-\beta)\epsilon}+1, \frac{\beta \epsilon}{T} \big)$-RDP for any $t=0,\ldots,T-1$. Then the composition theorem of RDP shows that Algorithm~\ref{alg:dp-sgd-3} satisfies $\big( \frac{\log(1/\delta)}{(1-\beta)\epsilon}+1, \beta \epsilon \big)$-RDP. Finally, by the relationship between RDP and $(\epsilon,\delta)$-DP, we have Algorithm~\ref{alg:dp-sgd-4} satisfies $(\epsilon, \delta)$-DP.     
\end{proof}

Next we take a look at the utility bound of \ref{alg:dp-sgd-4}. Let $\wbf^* = \arg\min_{\wbf \in \wcal} L(\wbf)$, the utility bound can be decomposed as follow
\[
L(\acal(S)) - L(\wbf^*) = L(\acal(S)) - L_S(\acal(S)) + L_S(\acal(S)) - L_S(\wbf^*) + L_S(\wbf^*) - L(\wbf^*).
\]
Taking expectation on both sides and noting that $\ebb[L_S(\wbf^*) - L(\wbf^*)] = 0$, we further derive
\[
\ebb[L(\acal(S)) - L(\wbf^*)] = \ebb[L(\acal(S)) - L_S(\acal(S))] + \ebb[L_S(\acal(S)) - L_S(\wbf^*)] .
\]

\begin{definition}
An (randomized) algorithm $\acal$ for pairwise learning is called $\epsilon_{\text{stab}}$-uniformly stable with $\epsilon_{\text{stab}} > 0$ if for all neighborhood datasets $S, S' \in \zcal^n$ we have
\[
\sup_{\zbf, \zbf' \in \zcal}\ebb_\acal[\ell(\acal(S);\zbf, \zbf') - \ell(\acal(S');\zbf, \zbf')] \leq \epsilon_{\text{stab}}
\]
\end{definition}

\begin{theorem}[Theorem 2 in \citet{shen2020stability}]
If algorithm $\acal$ for pairwise learning is $\epsilon_{\text{stab}}$-uniformly stable with $\epsilon_{\text{stab}} > 0$ then we have
\[
\big|\ebb_{S,\acal}[L_S(\acal(S)) - L(\acal(S))]\big| \leq \epsilon_{\text{stab}}
\]
\end{theorem}

\begin{theorem}
Suppose the function $L_S$ is convex. And
\begin{enumerate}
    \item[a)] suppose $\ell$ is $G$-Lipschitz continuous and $L$-smooth. Then Algorithm \ref{alg:dp-sgd-4} satisfies  \[\epsilon_{\text{stab}}(\bar{\wbf}_T) = \ocal\Big(\frac{\eta T}{n}\Big)\]
    \item[b)] suppose $\ell$ is $G$-Lipschitz continuous. Then Algorithm \ref{alg:dp-sgd-4} satisfies \[\epsilon_{\text{stab}}(\bar{\wbf}_T) = \ocal\Big(\eta\sqrt{T} + \frac{\eta T}{n}\Big)\]
\end{enumerate}
\end{theorem}

\begin{proof}
The proof is straight forward by noting the probability of picking the different example between $S$ and $S'$ at iteration $t$ is $\frac{2}{n}$.
\end{proof}

\begin{theorem}
Suppose the function $L_S$ is convex and $\ell$ is $G$-Lipschitz continuous. Then Algorithm \ref{alg:dp-sgd-4} satisfies
\[
L_S(\bar{\wbf}_T) - L_S(\wbf^*) = \ocal\Big(\frac{1}{\eta T} + \eta + \eta d\sigma^2\Big)
\]
By further noting 
\[
\sigma^2 = \ocal\Big(\frac{T\log(1/\delta)}{n^2\epsilon^2}\Big)
\]
under some assumption, we have
\[
L_S(\bar{\wbf}_T) - L_S(\wbf^*) = \ocal\Big(\frac{1}{\eta T} + \eta + \frac{\eta dT\log(1/\delta)}{n^2\epsilon^2}\Big)
\]
\end{theorem}

\begin{proof}
This proof is again straight forward by noting that $\nabla \ell(\wbf_t; \zbf_{i_t}, \zbf_{j_t})$ for fixed $\wbf_t$ is an unbiased estimator of $\nabla L_S(\wbf_t)$.
\end{proof}

\section{Privacy Guarantee}

\begin{lemma}
This lemma aims to track the privacy amplification by subsampling. It is a working progress. 
\end{lemma}

\begin{proof}
% Let $p_t, q_t$ de note the distributions $(\mcal\circ \code{subsample})_t(S), (\mcal\circ \code{subsample})_t(S')$, respectively, at iteration $t$. Let $E_t$ be the event such that the subsample includes the $n$th item at iteration $t$. Let $m_t$ be the number of $n$th sample being chosen by $\code{subsample}$ operation until iteration $t$. We have
% \begin{align*}
% p_t(\cdot| m_t) = \ebb_{E_t}[p_t(\cdot| E_t, m_t)] = \frac{1}{n}p_t(\cdot| E_t, m_t) + \Big(1 - \frac{1}{n}\Big) p(\cdot | E_t^c, m_t)    
% \end{align*}
% and
% \begin{align*}
% p_t = & \ebb_{m_t} [p_t(\cdot| m_t)] = \sum_{m_t = 0}^t{t \choose m_t}\Big(\frac{1}{n}\Big)^{m_t}\Big(1 - \frac{1}{n}\Big)^{t-m_t} p_t(\cdot|m_t)  \\
% = & \sum_{m_t = 0}^t{t \choose m_t}\Big(\frac{1}{n}\Big)^{m_t}\Big(1 - \frac{1}{n}\Big)^{t-m_t} \Big( \frac{1}{n}p_t(\cdot| E_t, m_t) + \Big(1 - \frac{1}{n}\Big) p(\cdot | E_t^c, m_t)\Big)
% \end{align*}
% Another way to display $p_t$ is as follow. 
Let $p_t, q_t$ de note the distributions $(\mcal\circ \code{subsample})_t(S), (\mcal\circ \code{subsample})_t(S')$, respectively, at iteration $t$. 

Recall in \citet{wang2019subsampled} that $E$ is defined as the event such that the subsample includes the $n$th item. Then the distribution $p = \mcal\circ \code{subsample}(S)$ can be expressed as
\[
p = \ebb_E[p(\cdot|E)] = \frac{1}{n}p(\cdot|E) + \Big(1 - \frac{1}{n}\Big) p(\cdot|E^c)
\]
which means $E$ follows a Bernoulli distribution with probability $\frac{1}{n}$. Let us firstly look at a coarse way to approach the pairwise learning problem by defining $F_t$ as the event such that $n$th item is included in the subsample until time $t$. Hence 
\[
\pbb[F_t^c] = \Big(1 - \frac{1}{n}\Big)^{t+1}
\]
and
\[
\pbb[F_t] = 1 - \Big(1 - \frac{1}{n}\Big)^{t+1}.
\]
Then the distribution $p_t$ can be expressed as 
\[
p_t = \ebb_{F_t}[p_t(\cdot|F_t)] = \Big(1 - \Big(1 - \frac{1}{n}\Big)^{t+1}\Big)p_t(\cdot|F_t) + \Big(1 - \frac{1}{n}\Big)^{t+1} p_t(\cdot|F_t^c)
\]
and 
\[
q_t = \ebb_{F_t}[p_t(\cdot|F_t)] = \Big(1 - \Big(1 - \frac{1}{n}\Big)^{t+1}\Big)q_t(\cdot|F_t) + \Big(1 - \frac{1}{n}\Big)^{t+1} q_t(\cdot|F_t^c)
\]
and by construction $p(\cdot|F_t^c) = q(\cdot|F_t^c)$. Substituting the observation into the ternary-$|\chi|^j$-divergence, we have
\begin{align*}
D_{|\chi|^j} (p_t, q_t || r_t) = & \ebb_{r_t} \Big[\Big(\frac{|p_t-q_t|}{r_t}\Big)^j\Big]   \\
= & \Big(1 - \Big(1 - \frac{1}{n}\Big)^{t+1}\Big)^j \ebb_{r_t} \Big[\Big(\frac{\big|p_t(\cdot|F_t) - p_t(\cdot|F_t)\big|}{r_t}\Big)^j\Big]\\
\leq & \Big(\frac{t+1}{n}\Big)^j \ebb_{r_t} \Big[\Big(\frac{\big|p_t(\cdot|F_t) - p_t(\cdot|F_t)\big|}{r_t}\Big)^j\Big]
\end{align*}
where the last inequality we used an elementary inequality $(1 - a)^x \geq 1 - ax$ for any $0<a<1$ and $x\geq 1$. As we can see the amplification rate $\frac{t+1}{n}$ is looser compare to $\frac{1}{n}$ in \citet{wang2019subsampled}. 

Similar to \citet{wang2019subsampled}, we need to define a new $\sigma$-field to redundantly represent subsampling over $[n-1]$ and $[n]$ under the same uniform probability measure while establishing a one-to-one mapping between pairs of events such that the corresponding index of the subsample differs by only one datapoint.

% We define $J$ be a random subset of size $t+1$ chosen by the \code{subsample} operator $t+1$ times. In addition, we define an auxiliary dummy variable $i \sim \text{Unif}(1, \cdots, t+1)$. Let $i$ be independent to everything else, so it is clear that $r(\cdot|J) = r(\cdot|J,i)$. In other words,
% \[
% r(\cdot) = \ebb_{J,i}[r(\cdot|J,i)] = \frac{1}{(t+1){n\choose t+1}} \sum_{J \subset [n], i \in [t+1]} r(\cdot|J).
% \]
% Now, define functions $g$ and $g'$ on index sex $J, i$ such that
% \begin{equation*}
% g(J,i) = \begin{cases}
% p(\cdot| J) & \text{if } n\in J\\
% p(\cdot| J \cup \{n\} \setminus J[i]) & \text{otherwise}
% \end{cases}
% \end{equation*}
% and
% \begin{equation*}
% g'(J,i) = \begin{cases}
% q(\cdot| J) & \text{if } n\in J\\
% q(\cdot| J \cup \{n\} \setminus J[i]) & \text{otherwise.}
% \end{cases}
% \end{equation*}
% Check that $p_t(\cdot| F_t) = \ebb_{J,i}[g(J,i)]$ 

Next we introduce a finer description of the distributions $p_t, q_t$. A natural extension of Bernoulli random variable $E$ is to define $E_t$ as the event such that the $n$th item is included in the subsample $m$ times until time $t$. Then the distribution $p_t$ can be expressed as 
\begin{align*}
p_t = \ebb_{E_t}[p(\cdot|E_t)] = \sum_{m=0}^{t+1} {t+1 \choose m} \Big(\frac{1}{n}\Big)^m \Big(1 - \frac{1}{n}\Big)^{t+1-m} p_t(\cdot| E_t = m) 
\end{align*}
which indicates $E_t$ follows a binomial distribution with probability $\frac{1}{n}$. Similarly, we have
\begin{align*}
q_t = \ebb_{E_t}[p(\cdot|E_t)] = \sum_{m=0}^{t+1} {t+1 \choose m} \Big(\frac{1}{n}\Big)^m \Big(1 - \frac{1}{n}\Big)^{t+1-m} q_t(\cdot| E_t = m)
\end{align*}
and by construction, $p_t(\cdot| E_t = 0) = q_t(\cdot| E_t = 0) $.

Substituting the observation into the ternary-$|\chi|^j$-divergence, we have
\begin{align*}
D_{|\chi|^j} (p_t, q_t || r_t) = & \ebb_{r_t} \Big[\Big(\frac{|p_t-q_t|}{r_t}\Big)^j\Big]   \\
= & \ebb_{r_t} \Bigg[\Bigg(\frac{\Big|\sum_{m=1}^{t+1} {t+1 \choose m} \Big(\frac{1}{n}\Big)^m \Big(1 - \frac{1}{n}\Big)^{t+1-m} \big(p_t(\cdot| E_t = m) - q_t(\cdot| E_t = m)\big)\Big|}{r_t}\Bigg)^j\Bigg]
\end{align*}
The goal here is to derive an $\Big(\frac{1}{n}\Big)^j$ amplification of some kind of ternary-$|\chi|^j$-divergence.

A third way to describe $p_t, q_t$ is by fixing the past sampling. Let $D_t$ be the random subset chosen by $\code{subsample}$ until time $t$ and $G_t$ be the event that $n$th item is chosen at time $t$. In this case, we have
\[
p_t = \ebb_{D_t, G_t}[p_t(\cdot|D_t, G_t)] = \ebb_{D_t}\Big[\frac{1}{n}p_t(\cdot|D_t, G_t) + \Big(1 - \frac{1}{n}\Big)p_t(\cdot|D_t, G_t^c)\Big]
\]

Now we take a new perspective to describe the distributions $p_t, q_t$. The main idea is to introduce the indicator function and utilize the subadditivity of the indicator function hoping to decouple the pairwise dependence. The distribution $p_t$ takes the form
\begin{align*}
p_t = & \frac{1}{t}\sum_{k=1}^t \nabla \ell(\wbf_t; z_{i_{t+1}}, z_{i_k}) + \ncal(0, \sigma_t^2I)    \\
= & \frac{1}{t}\sum_{k=1}^t \nabla \ell(\wbf_t; z_{i_{t+1}}, z_{i_k})\big(\ibb[i_{t+1}\neq n \wedge i_k\neq n] + \ibb[i_{t+1}= n \vee i_k=n]\big) + \ncal(0, \sigma_t^2I)
\end{align*}
Note that with probability $1-\gamma$, 
\begin{multline*}
\frac{1}{t}\sum_{k=1}^t\big(\ibb[i_{t+1}\neq n \wedge i_k\neq n] + \ibb[i_{t+1}= n \vee i_k=n]\big)
\leq \frac{1}{t}\sum_{k=1}^t\big(\ibb[i_{t+1}\neq n] + \ibb[i_{t+1}= n] + \ibb[i_k=n] \big)\\
\leq \ibb[i_{t+1}\neq n] + \ibb[i_{t+1}= n] + \frac{1}{n} + \frac{\log(1/\gamma)}{t} + \sqrt{\frac{\log(1/\gamma)}{tn}}.    
\end{multline*}
where in the first inequality we used the subadditivity of the indicator function and in the second inequality we used the Bernstein inequality for Bernoulli random variables.
\end{proof}

\section{A New Algorithm}

\begin{algorithm}[ht!]
\caption{Differentially Private Stochastic Gradient Descent for Pairwise Learning\label{alg:dp-sgd-2}}
\begin{algorithmic}[1]
\STATE {\bf Inputs:} Private dataset $S = \{\zbf_i: i=1,\ldots, n\}$, learning rates $\{\eta_t\}_{t=1}^T$, initial points $\wbf_1$, 
\STATE $F_1 = \emptyset, t=1$
\STATE Compute $\sigma^2 = \frac{7G^2T}{\beta n^2\epsilon}\Big(\frac{\log(1/\delta)}{(1-\beta)\epsilon} + 1\Big)$
\WHILE{$|F_t| \leq n$}
\STATE Select $i_{t+1}$ uniformly from $[n]$
\STATE Sample noise $\ubf_t \sim \ncal(0, \sigma^2 I)$
\IF{$i_{t+1} \in F$}
\STATE $\wbf_{t+1} = \proj_\wcal\big(\wbf_t - \eta_t \ubf_t\big)$
\STATE $F_{t+1} = F_t$
\ELSE
\STATE $\wbf_{t+1} = \proj_\wcal\big(\wbf_t - \frac{\eta_t}{|F_t|}\sum_{i_k \in F_t} \big(\nabla \ell(\wbf_t; \zbf_{i_{t+1}}, \zbf_{i_k}) + \ubf_t\big)\big)$
\STATE $F_{t+1} = F_t \cup \{i_{t+1}\}$
\ENDIF
\STATE $t = t + 1$
\ENDWHILE
\STATE {\bf Outputs:} $\bar{\wbf}_T$ to be specified
\end{algorithmic}
\end{algorithm}


We first introduce some notation. Let $\widehat{\mcal}_t: \wcal \times [n] \times \zcal^n \rightarrow \wcal \times [n]$ be  the mechanism which describes the $t$-th iteration of the algorithm. We are first going to show that the first coordinate of each $\widehat{\mcal}_t$ is sufficiently differentially private.

\begin{lemma}
If $\mcal$ is $(\epsilon, \delta)$-DP, then $\mcal\circ\code{subsample}$ obeys $(\epsilon',\delta')$-DP with $\epsilon' = \log(1+ \frac{1}{n}(\exp(\epsilon)-1))$ and $\delta'=\frac{\delta}{n}$.
\end{lemma}

\begin{proof}

Without loss of generality, we assume the different example between $S$ and $S'$ is the $n$-th item. We first consider the case $n \not\in F$. For fixed $\wbf, F$ and any measurable $\ecal \subseteq \wcal$ define the measures
\begin{align*}
A(\ecal) = & \pbb\big[\mcal(\wbf, F, S) \in \ecal| i_{t+1} = n, n \not\in F\big]	\\
A'(\ecal) = & \pbb\big[\mcal(\wbf, F, S') \in \ecal| i_{t+1} = n, n \not\in F\big]	\\
B(\ecal) = & \pbb\big[\mcal(\wbf, F, S) \in \ecal| i_{t+1} \neq n, n \not\in F\big]	\\
B'(\ecal) = & \pbb\big[\mcal(\wbf, F, S') \in \ecal| i_{t+1} \neq n, n \not\in F\big].
\end{align*}
We have
\begin{align*}
& \pbb\big[\mcal\circ\code{subsample}(\wbf, F, S) \in \ecal | n \not\in F\big] - \frac{\delta}{n} = \frac{1}{n} A(\ecal) + \Big(1 - \frac{1}{n}\Big) B(\ecal)  - \frac{\delta}{n}\\	
\stackrel{(a)}{\leq} & \frac{1}{n} \big(\exp(\epsilon) \min\{A'(\ecal), B(\ecal)\}\big) + \frac{\delta}{n} + \Big(1 - \frac{1}{n}\Big)B(\ecal) - \frac{\delta}{n}\\
= & \frac{1}{n} \big( \min\{A'(\ecal), B(\ecal)\} + (\exp(\epsilon) - 1) \min\{A'(\ecal), B(\ecal)\}\big) + \Big(1 - \frac{1}{n}\Big)B(\ecal) \\
\leq & \frac{1}{n} \Big( \min\{A'(\ecal), B(\ecal)\} + (\exp(\epsilon) - 1) \Big(\frac{1}{n}A'(\ecal) + \Big(1 - \frac{1}{n}\Big) B(\ecal)\Big)\Big) + \Big(1 - \frac{1}{n}\Big)B(\ecal) \\
\leq & \frac{1}{n} \Big(A'(\ecal) + (\exp(\epsilon) - 1) \Big(\frac{1}{n}A'(\ecal) + \Big(1 - \frac{1}{n}\Big) B(\ecal)\Big)\Big) + \Big(1 - \frac{1}{n}\Big)B(\ecal) \\
= & \Big(\frac{1}{n}A'(\ecal) + \Big(1 - \frac{1}{n}\Big) B(\ecal)\Big)\Big) + \frac{1}{n}(\exp(\epsilon) - 1) \Big(\frac{1}{n}A'(\ecal) + \Big(1 - \frac{1}{n}\Big) B(\ecal)\Big)\Big) \\
= & \Big(1 + \frac{1}{n}(\exp(\epsilon) - 1) \Big)\Big(\frac{1}{n}A'(\ecal) + \Big(1 - \frac{1}{n}\Big) B(\ecal)\Big)\Big) \\
\stackrel{(b)}{=} & \Big(1 + \frac{1}{n}(\exp(\epsilon) - 1) \Big)\Big(\frac{1}{n}A'(\ecal) + \Big(1 - \frac{1}{n}\Big) B'(\ecal)\Big)\Big) \\
= & \Big(1 + \frac{1}{n}(\exp(\epsilon) - 1) \Big)\pbb\big[\mcal\circ\code{subsample}(\wbf, F, S') \in \ecal | n \not\in F\big]
\end{align*}
where in (a) we used the fact that $A(\ecal) \leq \exp(\epsilon)A'(\ecal) + \delta$ and $A(\ecal) \leq \exp(\epsilon)B(\ecal) + \delta$ by the DP assumption. In particular, $A(\ecal) \leq \exp(\epsilon)B(\ecal) + \delta$ because the mechanism $\mcal(\wbf, F, S)$ in $B(\ecal)$ also follows the Gaussian distribution with the same noise. And in (b) we used $B(\ecal) = B'(\ecal)$ because the two mechanism follows the same distribution when $i_{t+1}\neq n, n\not\in F$.

Next we move on to the case $n \in F$. Again, for fixed $\wbf, F$ and any measurable $\ecal \subseteq \wcal$ define the measures
\begin{align*}
C(\ecal) = & \pbb\big[\mcal(\wbf, F, S) \in \ecal| i_{t+1} = n, n \in F\big]	\\
C'(\ecal) = & \pbb\big[\mcal(\wbf, F, S') \in \ecal| i_{t+1} = n, n \in F\big]	\\
D(\ecal) = & \pbb\big[\mcal(\wbf, F, S) \in \ecal| i_{t+1} \neq n, n \in F\big]	\\
D'(\ecal) = & \pbb\big[\mcal(\wbf, F, S') \in \ecal| i_{t+1} \neq n, n \in F\big].
\end{align*}
Note that in the pointwise learning setting, we automatically have $C(\ecal) = C'(\ecal)$ and $D(\ecal) = D'(\ecal)$. The first one holds since the mechanisms in $C$ and $C'$ are the same Gaussian mechanism. The second one holds as the gradient update only performs on the newly sampled index $i_{t+1}$ hence the mechanisms are again the same. In the pairwise learning setting, we have
\begin{align*}
& \pbb\big[\mcal\circ\code{subsample}(\wbf, F, S) \in \ecal | n \in F\big] = \frac{1}{n} C(\ecal) + \Big(1 - \frac{1}{n}\Big) D(\ecal) \\	
\stackrel{(a)}{\leq} & \frac{1}{n} C(\ecal) + \Big(1 - \frac{1}{n}\Big)\big(\exp(\epsilon) \min\{C(\ecal), D'(\ecal)\} + \delta\big) \\
= & \frac{1}{n} C(\ecal) + \Big(1 - \frac{1}{n}\Big)\big(\min\{C(\ecal), D'(\ecal)\} + (\exp(\epsilon) - 1) \min\{C(\ecal), D'(\ecal)\} + \delta\big)\\
\leq & \frac{1}{n} C(\ecal) + \Big(1 - \frac{1}{n}\Big)\Big(\min\{C(\ecal), D'(\ecal)\} + (\exp(\epsilon) - 1) \Big(\frac{1}{n}C(\ecal) + \Big(1 - \frac{1}{n}\Big) D'(\ecal)\Big) + \delta\Big) \\
\leq & \frac{1}{n} C(\ecal) + \Big(1 - \frac{1}{n}\Big)\Big(D'(\ecal) + (\exp(\epsilon) - 1) \Big(\frac{1}{n}C(\ecal) + \Big(1 - \frac{1}{n}\Big) D'(\ecal)\Big) + \delta\Big) \\
= & \Big(\frac{1}{n}C(\ecal) + \Big(1 - \frac{1}{n}\Big) D'(\ecal)\Big)\Big) + \Big(1 - \frac{1}{n}\Big)(\exp(\epsilon) - 1) \Big(\frac{1}{n}C(\ecal) + \Big(1 - \frac{1}{n}\Big) D'(\ecal)\Big)\Big) + \Big(1 - \frac{1}{n}\Big)\delta\\
= & \Big(1 + \Big(1 - \frac{1}{n}\Big)(\exp(\epsilon) - 1) \Big)\Big(\frac{1}{n}C(\ecal) + \Big(1 - \frac{1}{n}\Big) D'(\ecal)\Big)\Big) + \Big(1 - \frac{1}{n}\Big)\delta\\
\stackrel{(b)}{=} & \Big(1 + \Big(1 - \frac{1}{n}\Big)(\exp(\epsilon) - 1) \Big)\Big(\frac{1}{n}C'(\ecal) + \Big(1 - \frac{1}{n}\Big) D'(\ecal)\Big)\Big) + \Big(1 - \frac{1}{n}\Big)\delta \\
= & \Big(1 + \Big(1 - \frac{1}{n}\Big)(\exp(\epsilon) - 1) \Big)\pbb\big[\mcal\circ\code{subsample}(\wbf, F, S') \in \ecal | n \in F\big] + \Big(1 - \frac{1}{n}\Big)\delta
\end{align*}

% Therefore, the results only hold if we have the following decomposition
% \begin{multline*}
% \pbb\big[\mcal\circ\code{subsample}(\wbf, F, S) \in \ecal\big] = \Big(1 - \frac{1}{n}\Big)\pbb\big[\mcal\circ\code{subsample}(\wbf, F, S) \in \ecal | n \not\in F\big]\\
%  + \frac{1}{n}\pbb\big[\mcal\circ\code{subsample}(\wbf, F, S) \in \ecal\big| n\in F]
% \end{multline*}

As we can see from the above results, the privacy guarantee after amplification by subsampling is of the order $\Big(\ocal\Big(\frac{n-1}{n}\epsilon\Big), \ocal\Big(\frac{n-1}{n}\delta\Big)\Big)$. The key issue is the identity $D(\ecal) = D'(\ecal)$ no longer holds, instead we have
\[
D(\ecal) \leq \exp(\epsilon) D'(\ecal) + \delta
\]
This inequality multiplied with the probability $\frac{n-1}{n}$ will damage the amplification rate. Therefore, we need a finer description on $D(\ecal)$ and $D'(\ecal)$. Suppose there is an event $G$ such that
\[
D(\ecal) = \frac{1}{n}D(\ecal|G) + \Big(1 - \frac{1}{n}\Big) D(\ecal|G^c)
\]
and
\[
D(\ecal|G^c) = D'(\ecal|G^c)
\]
then we are done. 

Of course there is an another way by proving 
\[
D(\ecal) \leq \Big(1 + \frac{1}{n}(\exp(\epsilon) - 1)\Big) D'(\ecal) + \frac{\delta}{n}
\]
which means the amplification by subsampling effect has already happened on $D(\ecal)$. In this case we have not afraid of the probability $\frac{n-1}{n}$. 

Please be noted that the first method may lead to the same results if the event $G$ further satisfies the condition 
\[
D(\ecal|G) \leq \exp(\epsilon)D'(\ecal|G) + \delta
\]
% Let us consider applying the peeling argument. Suppose $F$ is an ordered set with size $m$ and the $n$th item is chosen at $k$th position of $F$. Let $G_j$ denote the set
% \[
% G_j = \{k \leq m|2^{j-1} \leq k < 2^j\}
% \]
% Then
% \begin{align*}
% D(\ecal) = & \pbb\big[\mcal(\wbf, F, S) \in \ecal| i_{t+1} \neq n, n \in F\big]\\
% = & \sum_{j=1}^\infty \pbb\big[\mcal(\wbf, F, S) \in \ecal| i_{t+1} \neq n, n \in F, k \in G_j\big]\\
% \leq & 
% \end{align*}
\end{proof}

The next algorithm adds noises to each individual gradient.

\begin{algorithm}[ht!]
\caption{Differentially Private Stochastic Gradient Descent for Pairwise Learning\label{alg:dp-sgd-3}}
\begin{algorithmic}[1]
\STATE {\bf Inputs:} Private dataset $S = \{\zbf_i: i=1,\ldots, n\}$, learning rates $\{\eta_t\}_{t=1}^T$, initial points $\wbf_1$, 
\STATE $F_1 = \emptyset, t=1$
\STATE Compute $\sigma^2 = \frac{7G^2T}{\beta n^2\epsilon}\Big(\frac{\log(1/\delta)}{(1-\beta)\epsilon} + 1\Big)$
\WHILE{$|F_t| \leq n$}
\STATE Select $i_{t+1}$ uniformly from $[n]$
\STATE Sample noises $\{\ubf_t^k\}$ such that $\ubf_t^k \sim \ncal(0, \sigma^2 I)$
\IF{$i_{t+1} \in F_t$}
\STATE $\wbf_{t+1} = \proj_\wcal\big(\wbf_t - \frac{\eta_t}{|F_t|}\sum_{i_k \in F_t} \ubf_t^k\big)$
\STATE $F_{t+1} = F_t$
\ELSE
\STATE $\wbf_{t+1} = \proj_\wcal\big(\wbf_t - \frac{\eta_t}{|F_t|}\sum_{i_k \in F_t} \big(\nabla \ell(\wbf_t; \zbf_{i_{t+1}}, \zbf_{i_k}) + \ubf_t^k\big)\big)$
\STATE $F_{t+1} = F_t \cup \{i_{t+1}\}$
\ENDIF
\STATE $t = t + 1$
\ENDWHILE
\STATE {\bf Outputs:} $\bar{\wbf}_T$ to be specified
\end{algorithmic}
\end{algorithm}

We need the following supporting lemmas. The first lemma is an elementary probabilistic statement on the sampling. 

\begin{lemma}
For any iteration $t$ of Algorithm \ref{alg:dp-sgd-3}, the following statement is true
\[
\pbb[n \in \{i_{t+1},i_k\}] = \frac{2}{n}
\]
\end{lemma}

\begin{proof}

\end{proof}

The second lemma tells us sum of mechanisms sharing same inputs satisfies $(\sum\epsilon, \sum\delta)$-DP if each of them is $(\epsilon, \delta)$-DP.

We leverage the notion of \Renyi differential privacy (RDP) \citep{mironov2017renyi} as accountant for DP loss. The definition of RDP is given as follow.

\begin{definition}[\Renyi Differential Privacy]
A (randomized) algorithm	 $\acal$ is called $(\alpha,\epsilon)$-RDP with order $1 < \alpha$ if for all neighboring datasets $S,S'$, the following holds
\[
D_\alpha(\acal(S)||\acal(S')) = \frac{1}{\alpha-1}\log \ebb_{\theta \sim \acal(S')}\Big[\Big(\frac{\acal(S)(\theta)}{\acal(S')(\theta)}\Big)^\alpha\Big] \leq \epsilon.
\]
\end{definition}

The conversion from RDP to DP is given as follow
\begin{lemma}[\citep{mironov2017renyi}]
If $\acal$ obeys $(\alpha, \epsilon)$-RDP, then $\acal$ obeys $(\epsilon + \log(1/\delta)/(\alpha-1), \delta)$-DP for all $0 < \delta < 1$.
\end{lemma}


Next we introduce our differentially private algorithm as below. This algorithm takes the average of two gradients $\nabla f(\wbf_{t-1}; \zbf_{i_{t}}, \zbf_{i_{t-1}}$ and $\nabla f(\wbf_{t-1}; \zbf_{i_{t-1}}, \zbf_{i_{t}})$ at each iteration $t$, and then perturbs the averaged gradient by Gaussian noise.

\begin{algorithm}[H]
\caption{Differentially Private Online Markov Pairwise Learning\label{alg:dp-markov}}
\begin{algorithmic}[1]
\STATE {\bf Inputs:} Private dataset $S = \{\zbf_i: i=1,\ldots, n\}$,  learning rates $\{\eta_t\}_{t=1}^T$, initial points $\wbf_0$
\STATE Compute $\sigma^2 = \frac{7G^2T}{\beta n^2\epsilon}\Big(\frac{\log(1/\delta)}{(1-\beta)\epsilon} + 1\Big)$
\FOR{$t=1$ to $T$}
\STATE Randomly select $\zbf_{i_{t}}$ where $i_t \sim \text{Unif}([n])$
\STATE Sample noise $\bb_t \sim \ncal(0, \sigma^2 I)$
\STATE {$\wbf_{t} =    \wbf_{t-1} - {\eta_t}\big(\big(\nabla f(\wbf_{t-1}; \zbf_{i_{t}}, \zbf_{i_{t-1}}) + \nabla f(\wbf_{t-1}; \zbf_{i_{t-1}}, \zbf_{i_{t}})\big)/2 + \bbf_t\big) $} 
\ENDFOR
\STATE {\bf Outputs:} $\bw_\pri=\bw_T$
\end{algorithmic}
\end{algorithm}

A key component in the study of privacy guarantee of SGD-type algorithms is privacy amplification by subsampling. Before we present the privacy amplification theorem for Algorithm \ref{alg:dp-markov} we need to clarify differences between the notion of sampling. In the differential privacy community, NoisySGD with \textit{sampling without replacement} \citep{wang2019subsampled} often means at any fixed iteration $t$, the \code{Subsample} operator takes $n$ data points and outputs a sample from the uniform distribution over all subsets of size $m \leq n$. This procedure also refers to \textit{uniform subsampling}. While in the machine learning community, SGD with \textit{sampling with replacement} often means at each iteration $t$, a sampling without replacement procedure is performed and then the sampled data points are put back for sampling in the next iteration. This procedure also refers to \textit{random selection} \citep{hardt2016train}. In the case of Algorithm \ref{alg:dp-markov}, at iteration $t$, we performs sampling without replacement by the size $m=1$, while the gradient also depends on the last iteration sampling without replacement result $\zbf_{i_{t-1}}$. In this case, we define an operator $\code{Subsample}_t: \zcal^n \rightarrow \zcal^2$ such that $\code{Subsample}_t(S) = \{\zbf_{i_t}, \zbf_{i_{t-1}}\}$.

In cooperation with the $\code{Subsample}$ operator, at each iteration of Algorithm \ref{alg:dp-markov}, we consider the mechanism $\mcal_{t, f, \wbf, \bbf}$ by gradient perturbation defined as $\mcal_{t, f, \wbf, \bbf}: \zcal^n \rightarrow \rbb^d$ such that 
\[
\mcal_{t, f, \wbf, \bbf}(S) = \sum_{i,j=1, i\neq j}^n \nabla f(\wbf_{t-1}, \zbf_i, \zbf_j) + \bbf_t.
\]
We shorthand $\mcal_t = \mcal_{t, f, \wbf,, \bbf}$ without any ambiguity. This mechanism coincides with the gradient perturbation on the empirical objective. i.e. $\mcal_t = \nabla F_S(\wbf_{t-1}) + \bbf_t$. The mechanism after subsampling $\mcal_t \circ \code{Subsample}_t: \zcal^n \rightarrow \rbb^d$ is therefore given as  
\[
\mcal_t\circ\code{Subsample}_t(S) = \big(\nabla f(\wbf_{t-1}; \zbf_{i_{t}}, \zbf_{i_{t-1}}) + \nabla f(\wbf_{t-1}; \zbf_{i_{t-1}}, \zbf_{i_{t}})\big) + \bbf_t.
\]

We are now ready to present our privacy amplification by subsampling theorem.

\begin{theorem}\label{thm:RDPsubsample}
Consider $\mcal_t: \zcal^n \rightarrow \rbb^d$, and $\code{Subsample}_t: \zcal^n \rightarrow \zcal$ in Algorithm \ref{alg:dp-markov}. For all integer $\alpha \ge 2$, if $\mcal$ satisfies $(\alpha, \epsilon(\alpha) )$-RDP, then $\mcal\circ\code{Subsample}_t$ satisfies $(\alpha, \epsilon'(\alpha))$-RDP for any iteration $t$, where 
\begin{multline*} 
\epsilon'(\alpha)) \leq \frac{1}{\alpha-1}\log\Big(1 + \Big(\frac{2n-1}{n^2}\Big)^2{\alpha \choose 2} \min\{4(e^{\epsilon(2)} - 1), e^{\epsilon(2)}\min\{2, (e^{\epsilon(\infty)} - 1)^2\}\} \\
+ \sum_{j=3}^\alpha \Big(\frac{2n-1}{n^2}\Big)^j {\alpha \choose j} e^{\epsilon(j-1)\epsilon(j)} \min\{2, (e^{\epsilon(\infty)} - 1)^j\}\Big).
\end{multline*}
\end{theorem}

The proof of Theorem~\ref{thm:RDPsubsample} is inspired by \citet{wang2019subsampled} yet more involving. The major difference is on how to quantify the privacy loss by subsampling in terms of ternary-$|\chi|^\alpha$-DP \citep{wang2019subsampled}, which is defined below.

\begin{definition}\label{def:ternaryDP}
We say that a randomized mechanism $\M$ satisfies $\zeta$-ternary-$|\chi|^\alpha$-DP if for all $\alpha\ge 1$:
\[ \sup_{S,S',S'' \text{mutually adjacent}} \Big( D_{|\chi|^\alpha}\big( \M(S),\M(S')\parallel \M(S'') \big) \Big)^{1/\alpha} \le \zeta(\alpha),\]
where $ D_{|\chi|^\alpha}\big( p, q \parallel r \big) = \ebb_{r}\big[\big| \frac{p-q}{r} \big|^\alpha\big] $ is called the ternary-$|\chi|^\alpha$-divergence (or ternary Pearson–Vajda divergence) 
\end{definition}


The next key lemma depicts the subsampling effect in terms of Ternary-$|\chi|^\alpha$-DP. Compare to the parallel result (Proposition 16) in \citet{wang2019subsampled}, our amplification rate is $\ocal\Big(\frac{2}{n}\Big)$ instead of $\frac{1}{n}$. This is due to the nature of pairwise objectives and our $\code{Subsample}$ operator. Note that the coefficient $2$ will note affect scale the Gaussian noise variance.

\begin{lemma}[Subsampling lemma for Ternary-$|\chi|^\alpha$-DP]\label{lem:ternary-subsample}
Suppose $f(\wbf,\zbf, \zbf) = 0$ for any $\wbf\in \wcal$ and $\zbf \in \zcal$. If a mechanism $\mcal$ satisfies $\zeta$-ternary-$|\chi|^\alpha$-DP, then the algorithm $\mcal\circ\code{Subsample}_t$ satisfies $\frac{(2n-1)\zeta}{n^2}$-ternary-$|\chi|^\alpha$-DP for any $t$.
\end{lemma}

The assumption $f(\wbf,\zbf, \zbf) = 0$ is mild and can be satisfied by many pairwise learning tasks. Such assumption is introduced to avoid violating the mutually adjacent condition in Definition \ref{def:ternaryDP}. We are now ready to present the proof.

Before we present the proof of Lemma \ref{lem:ternary-subsample}, we need a supporting lemma to characterize the convexity of the ternary-$|\chi|^\alpha$-divergence \citep{wang2019subsampled}.

\begin{lemma}
The bivariate function $f(x,y) = x^j/y^{j-1}$ is jointly convex on $\rbb_+^2$ for $j > 1$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:ternary-subsample}]
Let $S$, $S'$ and $S''$ be three datasets of size $n$. If they are mutually adjacent, then they must differ on the same data point. Without loss of generality, we assume the $\rho$-th data point is different. Let $p, q, r$ denote the probability distribution of $\mcal\circ\code{Subsample}_t(S)$, $\mcal\circ\code{Subsample}_t(S')$ and $\mcal\circ\code{Subsample}_t(S'')$, respectively.  
	
Let $J$ be the ordered set of the indices returned by $\code{Subsample}_t$, i.e. $J = \{i_t,i_{t-1}\}$. Let $E$ be the event such that the sampled dataset includes the $\rho$-th data point, i.e. $E = \{\rho \in J\}$. We can decompose its probability as follow
\begin{align*}
\pbb[E] &= \pbb[i_t=\rho,i_{t-1}\ne \rho]+\pbb[i_t\ne \rho, i_{t-1}=\rho] +\pbb[i_t=\rho,i_{t-1}=\rho] 	\\
		& = \pbb[i_t=\rho]\pbb[i_{t-1}\ne \rho]+\pbb[i_t\ne \rho]\pbb[ i_{t-1}=\rho] +\pbb[i_t=\rho]\pbb[i_{t-1}=\rho] 	\\
		& = \frac{1}{n} \frac{n-1}{n} + \frac{1}{n} \frac{n-1}{n} + \frac{1}{n} \frac{1}{n} = \frac{2n-1}{n^2}
\end{align*} 
where the second identity holds since $i_t$ and $i_{t-1}$ are independent. Then we can rewrite our distributions $p, q$ as 
\[ p(\theta)=p(\theta | E)\pbb(E) +  p(\theta | E^c)\pbb(E^c), \]
\[ q(\theta)=q(\theta | E)\pbb(E) +  q(\theta | E^c)\pbb(E^c) ,\]  
where $E^c$ be the complement event of $E$.  It is obvious that $p(\theta | E^c)=q(\theta | E^c)$. Therefore the ternary Liese–Vajda divergence can be written as 
\begin{align*}\label{eq:subsample-rate-ternary}
\EX_{\theta \sim r}\Big[\Big|  \frac{ p(\theta )-q(\theta ) }{r(\theta) } \Big|^\alpha  \Big] = & \Big(\frac{2n-1}{n^2}\Big)^\alpha\EX_{\theta \sim r}\Big[   \frac{| p(\theta| E)-q(\theta|E) |^\alpha}{r(\theta)^\alpha}    \Big] \numberthis
\end{align*} 


As in \citet{wang2019subsampled}, the key step is to re-define a $\sigma$-field to unify the distributions $p(\theta | E), q(\theta | E)$ and $r(\theta)$. Yet the construction in our case is novel. Indeed, in their algorithm, the $\code{Subsample}$ operator is a subsampling without replacement procedure for fixed $t$. Therefore they considered an unordered set $J'$ of size $m$ chosen by the $\code{Subsample}$ with auxiliary dummy variable $i \sim \text{Unif}([m])$. As defined above, we consider an ordered set $J = \{i_t,i_{t-1}\}$. of size $2$. We need to introduce two independent auxiliary dummy variables $i \sim \text{Unif}([2])$ and $k \sim \text{Unif}([n])$. Let $i,k$ be independent to everything else, so it is clear that $r(\theta|J) = r(\theta|J,i,k)$. In other words,
\[
r(\theta) = \ebb_{J,i,k}[r(\theta|J,i,k)] = \frac{1}{2nn^2}\sum_{J \subset [n]\times[n], i\in [2], k\in[n]} r(\theta|J) = \frac{1}{n^2}\sum_{J \subset [n]\times[n]} r(\theta|J).
\]
Now, define functions $g$ and $g'$ on index set $J, i, k$ such that
\begin{align*}
g(J,i,k) \!=\! \begin{cases}
p(\theta|J) & \text{if } \rho \in J\\
p(\theta|J \!\cup\!\{\rho\} \!\setminus\! J[i]) & {\text{if } \rho \!\not\in\! J, k \!=\! n}\\
p(\theta|\{\rho,\rho\}) & \text{otherwise }
\end{cases}, \quad
g'(J,i,k) \!=\! \begin{cases}
q(\theta|J) & \text{if } \rho \in J\\
q(\theta|J \!\cup\! \{\rho\} \!\setminus\! J[i]) & \text{if } \rho \!\not\in\! J, k \!=\! n\\
q(\theta|\{\rho,\rho\}) & \text{otherwise }
\end{cases}
\end{align*}
Check that $p(\theta|E) = \ebb_{J,i,k}[g(J,i,k)]$ and $q(\theta|E) = \ebb_{J,i,k}[g'(J,i,k)]$. By such construction, we augment $(n-1)(n-2)$ components from $p(\theta|J\cup\{\rho\} \setminus J[i], k)$ or $q(\theta|J\cup\{\rho\} \setminus J[i], k)$ if $\rho \not\in J$ and $k = n$ and $n-1$ component from $p(\theta|(\rho,\rho),k)$ or $q(\theta|(\rho,\rho),k)$ if $\rho \not\in J$ and $k \neq n$. Therefore we have
\[
(2n-1) + (n-1)(n-2) + n-1 = n^2
\]
components in $g(J,i,k)$ or $g'(J,i,k)$ while establishing a one-to-one mapping between pairs of events.  This trick allows us to write
\begin{align*}\label{eq:condition-ternary-dp}
\ebb_q\Big(\frac{|p(\theta|E) - q(\theta|E)|}{q(\theta)}\Big)^j = & \int   \frac{|p(\theta|E) - q(\theta|E)|^j}{q(\theta)^{j-1}} \mathrm{d}\theta\\
\leq & \int  \ebb_{J,i,k} \Big[\frac{|g(J,i,k) - g'(J,i,k)|^j}{q(\theta|J)^{j-1}}\Big] \mathrm{d}\theta\\
= & \ebb_{J,i,k}\ebb_q \Big[\Big(\frac{|g(J,i,k) - g'(J,i,k)|}{q(\theta|J)}\Big)^j\Big| J, i, k\Big]\\
\leq & \zeta(j)^j \numberthis
\end{align*}
The first inequality is due to Jensen's inequality and joint convexity of function $x^j/y^{j-1}$ on $\rbb_+^2$. The second identity is due to Fubini's Theorem. The last inequality holds because of two reasons. When $g(J,i,k), g'(J,i,k)$ and $q(\theta|J)$ are built on mutually adjacent datasets, we apply the assumption $\mcal$ satisfies $\zeta$-ternary-$|\chi|^\alpha$-DP. When the underlying datasets among $g(J,i,k), g'(J,i,k)$ and $q(\theta|J)$ are not mutually adjacent, this only happens when $g(J,i,k)$ is built on $\{\zbf_\rho, \zbf_\rho\}$ while $g'(J,i,k)$ is built on $\{\zbf'_\rho, \zbf'_\rho\}$. Note that $g(J,i,k), g'(J,i,k)$ are the same Gaussian distribution of the random variable $\bbf_t$ because of the assumption $f(\wbf, \zbf, \zbf) = 0$ for any $\wbf \in \wcal$ and $\zbf \in \zcal$. Therefore the ternary Pearson–Vajda divergence is $0 \leq \zeta(j)$. 

The proof is complete by combining \eqref{eq:subsample-rate-ternary} and \eqref{eq:condition-ternary-dp}.
\end{proof}



% We need some supporting lemmas from \citet{wang2019subsampled} to finish the proof of Theorem \ref{thm:RDPsubsample-2}.

% \begin{lemma}
% If a randomized mechanism $\mcal$ is $\xi$-binary-$|\chi|^\alpha$-DP, then it is $\zeta$-ternary-$|\chi|^\alpha$-DP for some $\zeta$ satisfying $\xi(\alpha)^\alpha \leq \zeta(\alpha)^\alpha \leq 4\xi(\alpha)^\alpha$.
% \end{lemma}

After the subsampling lemma for ternary-$|\chi|^\alpha$-DP being established, the rest of the proof is to convert the privacy loss for ternary-$|\chi|^\alpha$-DP to RDP via the technique in \citet{wang2019subsampled}, which is presented below for completeness.

\begin{proof}[Proof of Theorem \ref{thm:RDPsubsample}]
Rewrite \Renyi divergence via Binomial expansion,  we have
\begin{align*}
\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)}\Big)^\alpha\Big] = & 1 + {\alpha \choose 1}\ebb_{\theta\sim q}\Big[\frac{p(\theta)}{q(\theta)} - 1\Big] + \sum_{j=2}^\alpha {\alpha \choose j}\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)} - 1\Big)^j\Big]\\
= & 1 + \sum_{j=2}^\alpha {\alpha \choose j}\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)} - 1\Big)^j\Big],
\end{align*}
where in the second equality used $\EX_{\theta\sim q}\Big[ \frac{p(\theta)}{q(\theta)}-1 \Big]= \int p(\theta) \mathrm{d}\theta -1=0$.
Taking maximum we further derive
\begin{align*}
\max_{p, q}\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)}\Big)^\alpha\Big] \leq & 1 + \sum_{j=2}^\alpha  {\alpha \choose j} \max_{p,q,r} \ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)-q(\theta)}{r(\theta)}\Big)^j\Big] \\
\leq & 1 + \sum_{j=2}^\alpha  {\alpha \choose j}\Big(\frac{2n-1}{n^2}\Big)^j \zeta(j)^j.
\end{align*}
where in the first inequality we used $(p-q)/q$ is a special case of $(p-q)/r$ and in the second inequality we used Lemma \ref{lem:ternary-subsample}. The rest of the proof follows by bounding the ternary-$|\chi|^\alpha$-DP using RDP as in \citet{wang2019subsampled}.
\end{proof}

Another key property of RDP is its interpretable adaptive composition \citep{mironov2017renyi}. We restate such property in favor of Algorithm \ref{alg:dp-markov}.

\begin{lemma}\label{lem:compostion}
If $\mcal_{1}\circ\code{Subsample}_{1}:\Z^n \times \R  \rightarrow \R^d$ obeys $(\alpha, \epsilon_1)$-RDP, and $\mcal_2\circ\code{Subsample}_2:\Z^n \times \R \times  \R^d \rightarrow \R^d$ obeys   $(\alpha,\epsilon_2)$-RDP, then the machanism defined as $(\mcal_{1}\circ\code{Subsample}_{1},\mcal_2\circ\code{Subsample}_2)$ satisfies $(\alpha,\epsilon_1+\epsilon_2)$-RDP.
\end{lemma}



\begin{proof}
Let $h:\Z^n \rightarrow \R^d\times \R^d$ be the result of running $\mcal_{1}\circ\code{Subsample}_{1}$ and $\mcal_2\circ\code{Subsample}_2$ sequentially. Let $X, Y$ and $Z$ denote the distributions of $\mcal_{1}\circ\code{Subsample}_{1}$, $\mcal_2\circ\code{Subsample}_2$, and the joint distribution $(X,Y)=h(S)$. $X',Y'$ and $Z'$ are similarly defined if the input is $S'$, where $S$ and $S'$ are neighboring datasets.  
\begin{align*}
   &\exp[ (\alpha-1) D_\alpha(h(S) \parallel h(S') ) ]\\
   &= \int_{\R^d \times \R^d} Z(x,y)^\alpha Z'(x,y)^{1-\alpha} \mathrm{d}x \mathrm{d}y\\
   &=\int_{\R^d}\int_{\R^d} \big( X(x)Y(y|x) \big)^\alpha \big(X'(x)Y'(y|x)\big)^{1-\alpha} \mathrm{d}y \mathrm{d}x\\
   &=\int_{\R^d}  X(x)^\alpha X'(x)^{1-\alpha} \int_{\R^d}   Y(y|x)^\alpha    Y'(y|x)^{1-\alpha} \mathrm{d}y \mathrm{d}x\\
   &\le \int_{\R^d}  X(x)^\alpha X'(x)^{1-\alpha}   \mathrm{d}x \exp((\alpha-1)\epsilon_2)\\
   &\le \exp((\alpha-1)(\epsilon_1+\epsilon_2))
\end{align*}
where
\[ X(x)=\pbb(\bw_1=x) =\pbb( \big(\nabla f(\wbf_0; \zbf_{i_1}, \zbf_{i_0}) + \nabla f(\wbf_0; \zbf_{i_0}, \zbf_{i_1})\big) + \bbf_1=x )\]
\[ Y(y|x)=\pbb(\bw_2=y|\bw_1)=\pbb(\big(\nabla f(\wbf_1; \zbf_{i_2}, \zbf_{i_1}) + \nabla f(\wbf_{1}; \zbf_{i_{1}}, \zbf_{i_2})\big) + \bbf_2 =y |\bw_{1}).\]

\end{proof}


The algorithm is listed as below as Algorithm \ref{alg:dp-markov-2}.

\begin{algorithm}[H]
\caption{Differentially Private Online Markov Pairwise Learning\label{alg:dp-markov-2}}
\begin{algorithmic}[1]
\STATE {\bf Inputs:} Private dataset $S = \{\zbf_i: i=1,\ldots, n\}$,  learning rates $\{\eta_t\}_{t=1}^T$, initial points $\wbf_0$
\STATE Compute $\sigma^2 = \frac{7G^2T}{\beta n^2\epsilon}\Big(\frac{\log(1/\delta)}{(1-\beta)\epsilon} + 1\Big)$
\FOR{$t=1$ to $T$}
\STATE Randomly select $\zbf_{i_{t}}$ where $i_t \sim \text{Unif}([n])$
\STATE Sample noise $\bb_t \sim \ncal(0, \sigma^2 I)$
\STATE {$\wbf_{t} =    \wbf_{t-1} - {\eta_t}\big(\nabla f(\wbf_{t-1}; \zbf_{i_{t}}, \zbf_{i_{t-1}}) + \bb_t \big) $} 
\ENDFOR
\STATE {\bf Outputs:} $\bw_\pri=\bw_T$
\end{algorithmic}
\end{algorithm}


Let us consider mechanism when $\zbf_{i_{t-1}}$ is chosen. We say that $\mcal_t $ satisfies $(\epsilon,\delta)$-DP if for any neighboring datasets $S$ and $S'$ of size $n$ differ in $\rho$-th data point, and any $i_{t-1} \in [n]$, there holds \[ \pbb(\M_t(S,i_{t-1})\in O) \le \exp(\epsilon) \pbb(\M_t(S',i_{t-1})\in O) +\delta . \]
For any neighboring datasets $S$ and $S'$ of size $n$ differ in $\rho$-th data point, consider the following two cases. (1) If $i_{t-1}\ne\rho$, i.e., $z_{i_{t-1}}=z'_{i_{t-1}}$, then the $\ell_2$-sensitivity of $\sum_{i=1}^n \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}})$ is  
\[ \Delta_2=\Big\| \sum_{i=1}^n\big( \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}})   - \nabla f(\wbf_{t-1}, \zbf'_i, \zbf'_{i_{t-1}}) \Big\|_2 \le 2G.\]

If   $i_{t-1}=\rho$, i.e., $z_{i_{t-1}}\ne z'_{i_{t-1}}$, then the $\ell_2$-sensitivity of $\sum_{i=1}^n \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}})$ is  
\[ \Delta'_2=\Big\| \sum_{i=1}^n\big( \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}})   - \nabla f(\wbf_{t-1}, \zbf'_i, \zbf'_{i_{t-1}}) \Big\|_2 \le 2nG.\]
That is, with probability $\frac{n-1}{n}$, the $\ell_2$-sensitivity of $\sum_{i=1}^n \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}})$ is $2G$, and with probability $\frac{ 1}{n}$, the $\ell_2$-sensitivity of $\sum_{i=1}^n \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}})$ is $2nG$. Therefore, it's not straightforward to choose $\sigma^2$ such that $\mcal_{t, f, \wbf, \bbf}(S, i_{t-1} ) = \sum_{i=1}^n \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}}) + \bb_t $ satisfies $(\epsilon,\delta)$-DP.  If we take $\sigma^2\propto \Delta_2 \log(1/\delta)$, then $\M_t$ satisfies $(\epsilon,\delta')$- DP, where $\delta' \ge \frac{1}{n}+\delta$. It's too bad for privacy protection. If we set  $\sigma^2\propto \Delta'_2 \log(1/\delta)$, the noise is too large and the utility of $\M$ is unsatisfactory.

%\puyu{Problem: how to design the original random mechanism(without subsampling) such that satisfies DP?}


\bigskip

\iffalse
Therefore, at each iteration of Algorithm \ref{alg:dp-markov-2}, we consider the mechanism $\mcal_{t, f, \wbf, \bbf}$ by gradient perturbation defined as $\mcal_{t, f, \wbf, \bbf}: \zcal^{n} \times \R \rightarrow \rbb^d $ such that 
\[\mcal_{t, f, \wbf, \bbf}(S, i_{t-1} ) = \sum_{i=1}^n \nabla f(\wbf_{t-1}, \zbf_i, \zbf_{i_{t-1}}) + \bb_t
\]
We shorthand $\mcal_t = \mcal_{t, f, \wbf, \bbf}$ without any ambiguity. 
 %Given $\mcal_t$, the $\code{Subsample}_t$ operator in our case can be viewed as the sampling without replacement procedure, i.e. $\code{Subsample}_t: \zcal^n \rightarrow \zcal$ and $\code{Subsample}_t(S) = \{\zbf_{i_t}\}$. 

The mechanism after subsampling $\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big): \zcal\times \R \rightarrow \rbb^d  $ is therefore given as  
\[
\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big)= \nabla f(\wbf_{t-1}, \zbf_{i_t}, \zbf_{i_{t-1}}) + \bbf_t
\]

We say that $\mcal_t $ satisfies $(\alpha,\epsilon(\alpha))$-RDP if for any neighboring datasets $S$ and $S'$ of size $n$ differ in $\rho$-th data point, and any $i_{t-1} \in [n]$, there holds \[ D_{\alpha}\Big( \M_t(S,i_{t-1} ) \parallel \M_{t}(S',i_{t-1}) \Big) \le \epsilon(\alpha). \] 
We are now ready to present our privacy amplification by subsampling theorem.

\fi
We are now ready to present our privacy amplification by subsampling theorem.


\begin{theorem}\label{thm:RDPsubsample-2}
Consider $\mcal_t: \zcal^n\times \R \rightarrow \rbb^d $, and $\mcal_t\big(\code{Subsample}_t(S), i_{t-1}  \big): \zcal^n \times \R \rightarrow \R^d $ in Algorithm \ref{alg:dp-markov-2}. For all integer $\alpha \ge 2$, if $\mcal$ satisfies $(\alpha, \epsilon(\alpha) )$-RDP, then $\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big)$ satisfies $(\alpha, \epsilon'(\alpha))$-RDP for any iteration $t$, where 
\begin{multline*} 
\epsilon'(\alpha)) \leq \frac{1}{\alpha-1}\log\Big(1 + \frac{1+n }{n^2} {\alpha \choose 2} \min\{4(e^{\epsilon(2)} - 1), e^{\epsilon(2)}\min\{2, (e^{\epsilon(\infty)} - 1)^2\}\} \\
+ \sum_{j=3}^\alpha \frac{1+n^{j-1}}{n^{j}} {\alpha \choose j} e^{\epsilon(j-1)\epsilon(j)} \min\{2, (e^{\epsilon(\infty)} - 1)^j\}\Big).
\end{multline*}
\end{theorem}


\begin{lemma}[Subsampling lemma for Ternary-$|\chi|^\alpha$-DP]
Suppose $f(\wbf,\zbf, \zbf) = 0$ for any $\wbf\in \wcal$ and $\zbf \in \zcal$. If  a mechanism  $\mcal_t\big(S, i_{t-1}   \big)$ satisfies $\zeta$-ternary-$|\chi|^\alpha$-DP, then the algorithm $\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big)$ satisfies $\frac{(1+n^{j-1})^{1/j}}{n} \zeta$-ternary-$|\chi|^\alpha$-DP for any $t$.
\end{lemma}

\begin{proof}
Let $S$, $S'$ and $S''$ be three datasets of size $n$. If they are mutually adjacent, then they must differ on the same data point. Without loss of generality, we assume the $\rho$-th data point is different.
Let $p,q,r$ denote the probability distribution of $\M_t(S,i_{t-1}), \M_t(S',i_{t-1})$ and $\M_t(S'',i_{t-1})$,  $p' , q' , r' $ denote the probability distribution of $\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big)$, $\mcal_t\big(\code{Subsample}_t(S'), i_{t-1}   \big)$ and $\mcal_t\big(\code{Subsample}_t(S''), i_{t-1}   \big)$, respectively.  
Note that $\M_t(S,i_{t-1})$ satisfies $\zeta$-ternary-$|\chi|^j$-DP, then for any $i_{t-1}$, there holds
\[ \EX_{\theta\sim r}\Big( \Big| \frac{p(\theta)-q(\theta)}{r(\theta)} \Big|^j \Big) \le \zeta(j)^j.\]


To show $\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big)$ satisfies $\frac{(1+n^{j-1})^{1/j}}{n} \zeta$-ternary-$|\chi|^\alpha$-DP, it  suffices to estimate
  \begin{align}\label{eq:subsample-1}
 	&D_{|\chi|^j}\big(p'(\theta ),q'(\theta ) \parallel r'(\theta )\big)\nonumber\\
 	&= 
 	\EX_{\theta \sim r'}\Big( \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta )} \Big|^j \Big)\nonumber\\
 	&=\pbb( i_{t-1}\ne \rho )  \EX_{\theta \sim r'}\Big( \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta )} \Big|^j \Big| i_{t-1}\ne \rho \Big) +
 	\pbb(i_{t-1}= \rho  ) \EX_{\theta \sim r'}\Big( \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta )} \Big|^j \Big| i_{t-1}= \rho \Big)\nonumber\\
 	&=\frac{n-1}{n} \EX_{\theta \sim r'}\Big( \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta  )} \Big|^j \Big| i_{t-1}\ne \rho \Big) +
 	\frac{1}{n} \EX_{\theta \sim r'}\Big( \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta  )} \Big|^j \Big| i_{t-1}= \rho \Big).
 \end{align}
 


First, consider the case $i_{t-1}\ne\rho$. In fact, this case matches the setting  in \citep{wang2019subsampled} with subsampling rate $\gamma=\frac{1}{n}$, i.e., we fix $ i_{t-1} $ and subsample $ i_t \sim \text{Unif}[n]$. Therefore, if $\M$ is $\zeta$-ternary-$|\chi|^j$-DP,
 \begin{align}\label{eq:subsample-2}
 	\EX_{\theta \sim r'}\Big( \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta)} \Big|^j \Big|  i_{t-1}\ne \rho   \Big)\le \frac{1}{n^j}\zeta(j)^j
 \end{align}
 
 
Now, consider the case $i_{t-1}=\rho$. Note that
\begin{align}\label{eq:subsample-3}
&\EX_{\theta \sim r'}\Big(  \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta)} \Big|^j  \Big|  i_{t-1}=\rho   \Big)\nonumber\\
&=\pbb(i_{t}\ne \rho)  \EX_{\theta \sim r'}\Big(  \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta )} \Big|^j \Big| i_{t-1}=\rho, i_{t}\ne \rho   \Big) + \pbb(i_{t}= \rho) \EX_{\theta \sim r'}\Big(  \Big| \frac{p'(\theta )-q'(\theta )}{r'(\theta)} \Big|^j \Big| i_{t-1}=\rho , i_{t}= \rho  \Big)\nonumber\\
&\le \frac{n-1}{n} \zeta(j)^j, 
\end{align}
 where in the last inequality used the assumption $f(\bw,z,z)=0$ for any $\bw\in \W$ and any $z\in \Z$. 
Plugging \eqref{eq:subsample-2} and \eqref{eq:subsample-3} back into \eqref{eq:subsample-1}, we have
 \begin{align*}
 	 D_{|\chi|^j}\big(p'(\theta ),q'(\theta ) \parallel r'(\theta )\big) 
 	  \le \frac{n-1}{n}\big( \frac{1}{n^j}+\frac{1}{n} \big)  \zeta^j \le \big( \frac{1}{n^j}+\frac{1}{n} \big)  \zeta^j.
 \end{align*}
that is,
$\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big)$ is $\frac{(1+n^{j-1})^{1/j}}{n} \zeta$-ternary-$|\chi|^j$-DP.

\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:RDPsubsample-2}]
Rewrite the \Renyi divergence via Binomial expansion, we have
\begin{align*}
\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)}\Big)^\alpha\Big] = & 1 + {\alpha \choose 1}\ebb_{\theta\sim q}\Big[\frac{p(\theta)}{q(\theta)} - 1\Big] + \sum_{j=2}^\alpha {\alpha \choose j}\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)} - 1\Big)^j\Big]\\
= & 1 + \sum_{j=2}^\alpha {\alpha \choose j}\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)} - 1\Big )^j\Big],
\end{align*}
where in the second equality used $\EX_{\theta\sim q}\Big[ \frac{p(\theta)}{q(\theta)}-1 \Big]= \int p(\theta) \mathrm{d}\theta -1=0$.
Taking maximum we further derive
\begin{align*}
\max_{p, q}\ebb_{\theta\sim q}\Big[\Big(\frac{p(\theta)}{q(\theta)}\Big)^\alpha\Big] \leq & 1 + \sum_{j=2}^\alpha  {\alpha \choose j} \max_{p,q,r} \ebb_{\theta\sim r}\Big[\Big|\frac{p(\theta)-q(\theta)}{r(\theta)}\Big|^j\Big] \\
\leq & 1 + \sum_{j=2}^\alpha  {\alpha \choose j} \frac{1+n^{j-1}}{n^{j}} \zeta(j)^j.
\end{align*}
where in the first inequality we used $(p-q)/q$ is a special case of $(p-q)/r$ and in the second inequality we used Lemma \ref{lem:ternary-subsample}. The rest of the proof follows by bounding the ternary-$|\chi|^\alpha$-DP using RDP as in \citet{wang2019subsampled}.
\end{proof}

Now, we simplify Theorem~\ref{thm:RDPsubsample-2} for Gaussian mechanism. 
\begin{lemma}
Gaussian mechanism $\mcal_t\big(\code{Subsample}_t(S), i_{t-1}   \big)=\nabla f(\wbf_{t-1}; \zbf_{i_{t}}, \zbf_{i_{t-1}}) + \bb_t$, where $\bb_t\sim \mathcal{N}(0,\sigma^2\mathbf{I})$, satisfies $(\alpha,  \alpha (1+n^{j-1})^{1/j} / n \sigma^2)$-RDP given   $\sigma^2 \ge $ and $\alpha-1 \le \sigma^2 \log(1/)$
\end{lemma}
\begin{proof}

\end{proof}



A key property of RPD is its interpretable adaptive composition, which is given as follow.


\begin{lemma}[Composition theorem]
If $\mcal_{1}\circ\code{Subsample}_{1}:\Z^n \times \R  \rightarrow \R^d$ obeys $(\alpha, \epsilon_1)$-RDP, and $\mcal_2\circ\code{Subsample}_2:\Z^n \times \R \times  \R^d \rightarrow \R^d$ obeys   $(\alpha,\epsilon_2)$-RDP, then the machanism defined as $(\mcal_{1}\circ\code{Subsample}_{1},\mcal_2\circ\code{Subsample}_2)$ satisfies $(\alpha,\epsilon_1+\epsilon_2)$-RDP.
\end{lemma}



\begin{proof}
Let $h:\Z^n \rightarrow \R^d\times \R^d$ be the result of running $\mcal_{1}\circ\code{Subsample}_{1}$ and $\mcal_2\circ\code{Subsample}_2$ sequentially. Let $X, Y$ and $Z$ denote the distributions of $\mcal_{1}\circ\code{Subsample}_{1}$, $\mcal_2\circ\code{Subsample}_2$, and the joint distribution $(X,Y)=h(S)$. $X',Y'$ and $Z'$ are similarly defined if the input is $S'$, where $S$ and $S'$ are neighboring datasets.  
\begin{align*}
   &\exp[ (\alpha-1) D_\alpha(h(S) \parallel h(S') ) ]\\
   &= \int_{\R^d \times \R^d} Z(x,y)^\alpha Z'(x,y)^{1-\alpha} \mathrm{d}x \mathrm{d}y\\
   &=\int_{\R^d}\int_{\R^d} \big( X(x)Y(y|x) \big)^\alpha \big(X'(x)Y'(y|x)\big)^{1-\alpha} \mathrm{d}y \mathrm{d}x\\
   &=\int_{\R^d}  X(x)^\alpha X'(x)^{1-\alpha} \int_{\R^d}   Y(y|x)^\alpha    Y'(y|x)^{1-\alpha} \mathrm{d}y \mathrm{d}x\\
   &\le \int_{\R^d}  X(x)^\alpha X'(x)^{1-\alpha}   \mathrm{d}x \exp((\alpha-1)\epsilon_2)\\
   &\le \exp((\alpha-1)(\epsilon_1+\epsilon_2))
\end{align*}
where
\[ X(x)=\pbb(\bw_1=x) =\pbb( \big(\nabla f(\wbf_0; \zbf_{i_1}, \zbf_{i_0}) + \nabla f(\wbf_0; \zbf_{i_0}, \zbf_{i_1})\big) + \bbf_1=x )\]
\[ Y(y|x)=\pbb(\bw_2=y|\bw_1)=\pbb(\big(\nabla f(\wbf_1; \zbf_{i_2}, \zbf_{i_1}) + \nabla f(\wbf_{1}; \zbf_{i_{1}}, \zbf_{i_2})\big) + \bbf_2 =y |\bw_{1}).\]

\end{proof}

